Search Result Clustering in Collaborative Sound Collections

The large size of nowadays' online multimedia databases makes retrieving their content a difficult and time-consuming task. Users of online sound collections typically submit search queries that express a broad intent, often making the system return large and unmanageable result sets. Search Result Clustering is a technique that organises search-result content into coherent groups, which allows users to identify useful subsets in their results. Obtaining coherent and distinctive clusters that can be explored with a suitable interface is crucial for making this technique a useful complement of traditional search engines. In our work, we propose a graph-based approach using audio features for clustering diverse sound collections obtained when querying large online databases. We propose an approach to assess the performance of different features at scale, by taking advantage of the metadata associated with each sound. This analysis is complemented with an evaluation using ground-truth labels from manually annotated datasets. We show that using a confidence measure for discarding inconsistent clusters improves the quality of the partitions. After identifying the most appropriate features for clustering, we conduct an experiment with users performing a sound design task, in order to evaluate our approach and its user interface. A qualitative analysis is carried out including usability questionnaires and semi-structured interviews. This provides us with valuable new insights regarding the features that promote efficient interaction with the clusters.

==> ICMR 20 - Search Result Clustering in Collaborative Sound Collections(1)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> ICMR 20 - Search Result Clustering in Collaborative Sound Collections(1)/S1_intro.tex <==
% retrieving sounds
Sounds used in movies, video-games, music and other media often originate from sound collections.
Thanks to online sharing platforms, a wide variety of content can be easily and freely shared.
In these platforms, the collection is generated by its users instead of coming from professional studios.
This results in non-uniformly-annotated content compared to professional libraries, which involve experts for annotating and organizing the collections~\cite{font2018sound}.
Therefore, browsing collaborative online sound collections is more arduous.
% often arduous.
% FFONT comment:
% this is fine, but I would argue that the fact that browsing the collections can be an arduous task* is not only because there is no uniform metadata, browsing professional libraries can also be arduous. and in fact the clustering strategies would be useful in both cases. If you see an easy way to mention that it would be nice to pose it in this more positive way. In other words, It is not that we're fixing a problem because user genrated content is "badly annotated", it is that we're making a technique to improve browsing sound collections which is useful for both professional libraries and user genrated content, and specially interesting in the latter as traditional browsing might be limited by the lack of metadata.

% search engines
Typically, users interact with these collections by using text-based search engines.
The primary role of these retrieval systems is to support users in accessing relevant content corresponding to their needs.
% or a document that satisfies an information need.
% The relevancy of results depend a lot on the specific use-case, which is not reflected from the query that the user submitted to the search engine.
%
% For musical content, people often consume music in the sharing platform itself, denoted as the \textit{read only} culture~\cite{lawrence2008remix}.
% In sound collections, user not only consume the content in the platform, but reuse it for a specific task or even create new content, which is denoted as the \textit{read/write} culture.
%
% query is ambiguous
After entering a text query, a user often faces a long list of results.
In the absence of specific query terms, the system may be unable to differentiate the relevance of the retrieved sounds to the user, whose needs are often very precise and related to highly-specialised tasks.
The user might be looking for audio clips with distinctive and detailed characteristics that can be represented by a wide range of proprieties.
In sound design, for instance, a user could be searching for a door closing sound which has a grinding noise that fits well with the movie ambiance and the visual aspect of the door.
In the case of music creation, they may be interested in finding instrument loops playing in a certain tonality, at a specific tempo and with different timbres.
%
In order to locate sounds of interest, the user usually needs to check the results one by one, listening to some of them and judging their relevance.
The process of finding the most appropriate sounds for specific user needs can be very time consuming and can fail in retrieving some sounds of interest when interacting with huge collections.
% what can the users tipically do

Users can narrow down the search by reformulating their queries, or by using some facet-based and tag-based filters~\cite{tunkelang2009faceted}.
When available, a user might find it very informative to explore the text and tags accompanying the sounds in the results page, in order to identify new terms for reformulating the query.
%
Tag clouds that organise and display popular tags from the results are particularly useful for that purpose. The user can quickly find particular sub-topics present in the search results~\cite{sinclair2008folksonomy}.
%
Nonetheless, functionalities based on textual metadata depend critically on the quality of the annotations, which is often limited in collaborative collections.
For this reason, content-oriented methods that are based on the audio content itself have increased potential in the development of novel approaches to navigate search results in such collections.

% It is interesting to see how the music retrieval systems have evolved and how music recommendation systems are now an important tool for people to explore music collections.
% These systems generally use information about the users’ listening behavior and historical ratings to estimate the user taste and recommend relevant musical pieces \cite{song2012survey}.
% In sound design, the task of creating an acoustic scene using sounds from audio collections is very specific, and does not depend only on the text query or more generally on his behaviors in the platform. 
% Moreover, the relevancy of a sound does not depend on the user tastes, or at least his personal preference is not the main concern. 
% A sound designer might look for footstep sounds over a particular surface and with a certain speed and strength.
% He might transform the content, by cutting, duplicating, mixing, applying audio processing effects, and finally end up with a convincing audio scene.
% %
% Recommending sounds seems complicated, since the user has a need that comes from his specific task in its specific context that is not easily reflected from his queries and more generally his behaviors in the platform. 
% Therefore the task of recommending relevant sounds to a user is complicated. 

% Specific task
% Sound retrieval often comes from a specific content need, which makes it difficult for traditional search engine ranking system to access the relevancy of the items in the collection.
% therefore, users might benefit from more sophisticated and specialized ways of accessing resources that fit their specific need.
% For instance, in the context of sound design, a user needs footstep sounds that fit well the video content he has to sonify.
%
% Retrieving such specific content poses a very challenging problem to the user and the sharing platform.

% Browsing results is time demanding
% Another important aspect of sound retrieval is that the user has to listen to the retrieved sounds in order to judged their relevancy, or even test it in context to be able to assess if the sound is good enough. 
% This makes the process of finding desired sound resources very costly compared for instance to images, where a user can instantaneously see the results.

% Search Result Clustering
% In response to a query, users have to face a list of results ranked in order of relevance to the query.
% The user starts at the top of the list and examine one result at a time, until she satisfies her need.
% For broad or ambiguous query, the results on different subtopics or meanings will be mixed together in the ranked list.
% It implies that the user have to go through a large number of irrelevant items to finally locate the one of interest.
%On the other hand, 
To that end, one complementary feature that search engines can incorporate is Search Result Clustering, which consists of grouping the results into different labeled clusters or categories.
It enables the user to enter a weakly-specified query and then explore the different themes that have been automatically extracted from the query results.
Clustering engines can complement the search by providing a faster way to retrieve relevant items, facilitating topic exploration and preventing the overlook of information~\cite{carpineto2009survey}.
However, such systems depend on more than just the clustering algorithm.
In order to guide the user to locate relevant items in the different clusters, meaningful labels should be assigned to each of them.
Moreover, the clustering has to be performed online within a short response time, requiring high computational efficiency.
Finally, the clustering engine requires a graphical user interface that provides an intuitive way to navigate the clusters, e.g. by conveying visual information.
%There are a lot of different approach for proposing a clustering engine for web documents \cite{carpineto2009survey}.


% OUTLINE OF THE PAPER
% TODO: REPHRASE AND EXTEND
In this work, we present the development of an audio-based Search Result Clustering engine that integrates with the Freesound website~\cite{font2013freesound}. 
% ADD CONTRIBUTION OF THE PAPER
In Section 2, we provide an overview of the related work from the literature. 
We then introduce our graph-based clustering approach and our interface in Section 3.
In section 4, we compare the performance of different features taken from the literature, by using sound metadata and ground-truth labels from manually-annotated datasets.
% Section 5 presents a qualitative evaluation on a few selected clustering examples.
% exposes?
Section 5 exposes an evaluation of the system with users performing a sound design task, which allows us to identify the key features that would enable the user to efficiently interact with the obtained clusters.
We end the paper with a conclusions section and discussion about future work.
% MAYBE REMOVE ABOUT FUTURE WORK? OR ADD FUTURE WORK IN CONCLUSION SECTION
% We finally conclude the paper in the last section.

==> ICMR 20 - Search Result Clustering in Collaborative Sound Collections(1)/S2_related_work.tex <==
% Content based search
% Text is the original and still most promising type of content of the web.
% When the accompany text description 
% However, there are several problems with using textual descriptions in unstructured, user-contributed sound databases for sound retrieval. 
% In collaborative multimedia collections, having unstructed 

%For instance social tags are often incomplete and inconsistent (find ref or reformulate!).
% This motivates the use of
In order to be able to organize and retrieve a large amount of poorly labeled data, automatic annotation methods have been extensively addressed in the research community.
% In order to be able to retrieve poor labeled data which miss extensive tags or textual descriptions, content-based methods have extensively addressed in the research community [REF].
The main requirement of these content-based approaches is a reliable numerical feature that can represent the content. 
These features were originally developed by carefully designing low-level descriptors by relying on domain knowledge about the sound class invariances.
% Some are derived directly from the time domain audio representation. For instance, the zero crossing rate allows the differentiation of periodic sounds, including musical instrument notes and noisy sounds such as ocean wave~\cite{peeters2011timbre}.
% spectral features
% Other features are derived from some spectral representations of the sounds and are mostly motivated by the fact that human perception widely relies on the frequency content of sound signals.
Some are derived directly from the time domain audio representation, whereas others use a spectral representations of the sounds which is mostly motivated by the fact that human perception widely relies on the frequency content of sound signals. 
Combining these different types of features enables the representation of the timbre of musical instruments or more high-level characteristics such as music moods and genres~\cite{peeters2011timbre, herrera2003automatic, kim2010music, eronen2000musical, tzanetakis2002musical}.
% A great example showing the potential of feature engineering is the mel-frequency cepstral coefficients (MFCCs) feature, which were inspired by the human voice production mechanism and its auditory perception. %[ref?]
% These coefficients allow a compact representation of the spectral envelope, that can efficiently represent a component of instruments' timbres~\cite{herrera2003automatic}, or more high-level features such as music mood~\cite{kim2010music}.
% However, this type of spectral features do not convey temporal dynamics of the sound~\cite{herrera2003automatic}. 
% By complementing them with temporal features they can provide good performances for instrument classification tasks~\cite{eronen2000musical}.
% For music content, aspects related to the instrumentation, rhythmic structure and harmonic content can characterize specific music genres~ \cite{tzanetakis2002musical}.
% %
% Harmony can be represented using chroma features, which is robust to variation in timbre and thus allow to capture harmonic progressions independently from the instruments used \cite{muller2010towards}.

Recently, techniques using Artificial Neural Networks have been able to provide an alternative to the handcrafted features previously developed. 
Tasks, such as auto-tagging or classification can be performed directly from the raw audio~\cite{pons2017end}, or using a spectrogram representation~\cite{hershey2017cnn}.
The internal representation that neural networks learn on one task, can be used for other applications~\cite{choi2017transfer}.
These transfer learning approaches make use of pre-trained models as a starting point for different tasks.
First layers from trained neural networks often learn similar features which can be applicable for many datasets and tasks~\cite{yosinski2014transferable}.
Intermediate layers can serve as a higher-level representations which can be used for clustering~\cite{jansen2017large}.


% Content-based methods for retrieving multimedia content in large collaborative collections is very promising, since it does not requires high quality tags or descriptions.

% There are many attempts on using content-based features for retrieving content \cite{yu2016strategies, doulaverakis2006hybrid, haque2013analysis, roma2010content, esmaili2004content, cano2006content, slaney2002semantic, slaney2002mixtures, wold1996content}. % TODO: remove some references
% In content-based methods, the media is retrieved and/or ranked using features derived from the content itself. 
% It has the advantage for instance to be able to retrieve poor labeled data for the which the content creator did not provide a precise textual description.
% There are two main kinds of methods based on acoustic features, some aim to propose a meaningful descriptor vector that can reflect proprieties of the sounds, and other try to assign high-level concepts with the use of classifiers for instance.
%

% Content based clustering
% TODO: introduce well clustering here. Maybe talk a bit more about features before.
Clustering is a type of unsupervised classification which consists in organising similar objects in groups called clusters.
Regardless of the clustering method, the content similarity measure involved is fundamental to the definition of a cluster.
This similarity notion is often derived from a feature space, on which a numerical distance or similarity is calculated.
When clustering audio content, the features and distance measures are often chosen carefully for a given specific task~\cite{black1997automatically, martins2007polyphonic, niessen2013hierarchical}.
However in the context of large online collections, the content is very diverse, containing speech, musical or environmental sounds.
This makes the choice of features and distance metric even more challenging.
%
Among the different approaches for clustering~\cite{fahad2014survey, xu2015comprehensive}, in the context of multimedia documents, density-based algorithms such as graph-based clustering methods are particularly well designed for dealing with computational efficiency and the heterogeneous aspect of the data~\cite{petkos2017graph}.
Moreover, in the context of sounds, graph-based algorithms based on k-Nearest Neighbors have been shown to be scalable and able to adapt to areas of different densities~\cite{roma2015algorithms}. 

% % Interfaces
% % REMOVE THAT AND ADD MORE INFO FROM LINTERATURE; CHECK GOOGLE DOC
% Human Computer Interaction research is an important area of research. 
% Graphical user interfaces enable the creation of powerful tools that combine human and machine capabilities.
% Existing works emphasized on automatic algorithms and are rarely concerned with how users can interact with these algorithms.
% However, human computer interaction is a very important aspect in the creation of effective systems.
% %
% Most of the tools used by sound designer and musicians offer limited capabilities for browsing large collections of audio files. 
% Digital audio workstations typically use only filenames and sometimes some forms of tag to explore personal collections of sounds.
% Professional collections are grouped by type and structured with handcrafted organization of concepts which may allow text-based retrieval method to be efficient enough.
% In the case of online large sound collections, search engines using text queries are often used, taking advantage of the accompany description of the content which the author provided.
% % tag cloud
% Tag clouds have been introduced and provide to users a valuable visual interface to browse web collections~\cite{hassan2006improving}. 
% They list the most popular tags present in the data collection and allow to construct queries by selecting tags. 
% Even if tags are sometimes disorganized due to their personal and subjective origin, they directly reflect the vocabulary of users, enabling matching users' real needs and language.
% % We believe that they can be complemented with a fixed vocabulary of concepts.

% % faceted search
% Faceted search allow to browse the collection in a multi-step refinement process by selecting categories, proprieties, attributes or characteristics of the content \cite{fagan2010usability}.
% Using facets to structure the information is not new and they are often used for providing a powerful interface for browsing collection using metadata.
% %Moreover, it is possible to conceptualise user tags by combining folskonomies with ontologies,
% % ABOUT COMBINING FOLKSONOMIES AND ONTOLOGIES FOR DISAMBIGUATING TAGS. Allow categorization of tags into information facets which are relevant in the audio domain (ref Fred Ontology based Tag recommendation)
% However, we do not find so many application using audio related information obtained by content-based analysis in the context of sound retrieval.
% % Facets look quite adequate to take advantage of the numerous automatic classification tools that have been proposed in the research community.

% visualisation and exploration
Signal processing approaches and machine learning techniques have been employed for organising and visualising large amounts of audio content~\cite{neumayer2005content, fallgren2018tool, wongsuphasawat2015voyager, tzanetakis2001marsyas3d}.
These techniques often make use of a dimensionality reduction technique over numerical features, and project the content into a 2-dimensional space where similar sounds are close from each other.
The user can locate a sound of interest and then explore its neighborhood.
For instance, spaces conveying timbral characteristics of the sounds enable quick exploration of collections~\cite{tzanetakis2001marsyas3d}.
The use of visualisation tools in browsing systems have been shown to facilitate and encourage broader exploration~\cite{wongsuphasawat2015voyager}.
%
Clustering can be used in this space in order to automatically extract groups of similar sounds or music~\cite{neumayer2005content}.
However, to our knowledge, this is the first study describing the integration of a sound clustering algorithm in a search engine. 
% integrating a clustering algorithm in a sound search engine has not been investigated or implemented yet.


% % DESCRIPTOR VISUALIZATION
% Other kind of interfaces propose to use visual characteristics to communicate informations about the sound sources.
% For instance, inspection of retrieved result can be done in a 2D or 3D timbral space (visual representation of large audio collections), like in \textit{TimbreSpace} \cite{tzanetakis2001marsyas3d}, a content and context aware visualization of audio
% collections where shape, color and position of objects are based on audio features. 
% It allows to quickly explore a collection of sounds whereas \textit{TimbreGrams} \cite{tzanetakis2000audio} allows to visualize variation of sound characteristics within one audio file. 
% It incorporates segmentation techniques and uses colors to depict timbral and temporal informations about the sound.

% NEED MORE SOTA FOR RECENT SEARCH INTERFACES

==> ICMR 20 - Search Result Clustering in Collaborative Sound Collections(1)/S3_proposed_approach.tex <==
\begin{figure}
 \centering
 \includegraphics[width=\columnwidth]{src_graph2.png}
 \caption{Diagram representing the steps of our clustering engine.}
 \label{fig:src_graph}
\end{figure}

Our clustering engine consists of several steps illustrated in Figure~\ref{fig:src_graph}. 
After collecting the results retrieved by the user's query, (i) nearest neighbor searches are computed for the top ranked results, (ii) a K-Nearest Neighbors graph is created, (iii) a community detection algorithm assigns each sound to one cluster with possible extra refinements, (iv) and finally the results are displayed with a visualisation.
The method is available as a service and its integration within the Freesound search engine is currently under development.
The code is available at this repository: \url{http://omitted.for.blind.review}.
We describe the audio features we will be using and comparing (Section 3.1), the graph-based clustering method (Section 3.2), a refinement strategy for discarding inconsistent clusters (Section 3.3) and the user interface of the system (Section 3.4).


\subsection{Audio Features}
% Our system can take any kind of feature as input. 
In this work, we compare the performance of our clustering method using three different sets of features. One set of manually selected features motivated from the literature (F1)~\cite{peeters2011timbre, herrera2003automatic, kim2010music, eronen2000musical, tzanetakis2002musical}, another set contains all of the lowlevel features available from the Essentia Freesound Extractor (F2)~\cite{bogdanov2013essentia}, and the third one uses embeddings from a neural network model trained on AudioSet~\cite{hershey2017cnn, gemmeke2017audio} (F3).
Table \ref{tab:features} details the different features.


% Most of these features are computed at a frame-based level. 
Most of the traditional acoustic features (F1, F2) are computed on frames of approximately 50 ms.
These frame-based features are summarised into a single feature vector, which ignores the temporal order.
% An aggregation of these frame-based features is then perform using a standard statistical methods which
It includes minimum and maximum values, mean and variance of the direct features and of their first and second derivatives.
The rest of the features, e.g. \textit{logattacktime}, consist of a single numerical value for an entire audio clip.
A dimentionality reduction is then performed using Principal Component Analysis over the entire sound collection, to reduce these concatenated statistics and values into a feature vector with 100 dimensions.
% These concatenated statistics are then reduced into a 100-sized feature 
% using Principal Component Analysis performed over the entire Freesound collection (from February 2019)~\cite{pearson1901liii}.
%
The deep neural network embeddings (F3) are calculated on windows of approximately 1 second.
These frame-based features are then aggregated with the mean statistic only.
% since many sounds do not contain many feature frame (we focus on clustering sounds with duration that varies from 0 to 10 seconds).
%

% TABLE FEATURES
\setlength{\tabcolsep}{0.3em}
\begin{table}
\small
 \begin{center}
 \begin{tabular}{c|l}
  \toprule
  Feature sets & Features \\
  \midrule
  \multirow{7}{*}{F1} & spectral centroid / complexity / spread / energy \\
  & energyband high / skewness /flatness db / rolloff, \\
  & temporal decrease / spread / kurtosis / skewness / \\
  & centroid, logattacktime, strongdecay, \\
  & effective duration, zerocrossingrate, \\
  & tristimulus, mfcc, dissonance \\
  \\
  \multirow{2}{*}{F2} & lowlevel features from the Essentia Freesound Extractor \\
  & \url{https://freesound.org/docs/api/analysis_docs.html} \\
  \\
  \multirow{2}{*}{F3} &  embeddings from AudioSet pre-trained model \\
  & \url{https://git.io/fjqsV} \\
  \bottomrule
 \end{tabular}
\end{center}
 \caption{The different features compared in this work.}
 \label{tab:features}
\end{table}

\subsection{Graph-Based Clustering}

Instead of directly using the features as input of a clustering method, we construct an intermediate representation of the data using a k-Nearest Neighbor Graph~\cite{dong2011efficient}. 
Each vertex represents a sound, and undirected edges connect each sound to its $k$ most similar according to the euclidean distance.
Some preliminary empirical tests made us choose $log2(N)$ for the value of $k$, where $N$ is the number of elements to cluster.
This allows us to reach a sufficient number of neighbors for small collections, while limiting it for larger collections, which ensures low-computational complexity.
Then, we use a community detection algorithm based on modularity optimisation for finding a partition of the graph~\cite{blondel2008fast}.
%
There are several reasons why we use such an approach. 
First it has been shown to be able to find clusters of different densities~\cite{roma2012factors}.
Second, the number of clusters does not need to be specified.
Also, it can take advantage of nearest neighbors search techniques that can be fast to compute (e.g. \cite{cayton2008fast} or similar approximate methods~\cite{aumuller2019ann, indyk1998approximate}).
In our work we use the Gaia library for performing nearest neighbor searches (\url{https://github.com/MTG/gaia}).
%
Another advantage of these graph-based methods is their simplicity which allows to use some interpretable heuristics for modifying the graph or its partition like discarding clusters of low quality.

\subsection{Discarding low quality clusters}

The amount of intra-cluster and inter-cluster edges (which are related to the modularity definition~\cite{newman2004finding}) can be used for defining an internal quality metric which is only based on data used by the clustering algorithm. 
Since we use the same data representation for the quality metric and for the clustering algorithm, it is not clear if it can be used for automatically assessing the quality of a cluster in terms of compactness and distinctiveness.
% TODO: explain better
In this work, we are interested in investigating its use as a confidence score for quantising the quality of an individual cluster, and possibly discard low quality clusters that should not be presented to the user in the context of Search Result Clustering.
% reflecting compactness and separation performances per cluster.
Our confidence score $c$ of a cluster ranges from 0 to 1 and is defined as following:
\begin{equation}
c = \frac {number \ of \ intra \ cluster \ edges} {total \ number \ of \ inter \ \& \ intra \ cluster \ edges}
\end{equation}
This confidence score will be higher for clusters that are more coherent, i.e., the sounds within a cluster are more similar to sounds within the same cluster than to sounds from other clusters.
In the case that many of the elements of a cluster have edges to elements of other clusters, this score will be lower.
This score penalises clusters that are not compact and distinct from other clusters.
In this work, we investigate the use of this simple internal metric (which does not make use of any external knowledge about the data) as a confidence measure for discarding potentially irrelevant clusters.

\subsection{User Interfaces}
% EXPLAIN OUR INTERFACES
% TRADITIONAL FACET SEARCH
% 2D Visualisation
To allow the user to interact with the clusters, we propose two different interfaces.
One consists of a traditional facet filtering approach, where the user can apply filters on the result to display only sounds from one cluster. Figure \ref{fig:src_facet} shows the modified Freesound search interface with the added clusters facets.
Three labels are displayed for each cluster which correspond to the most occurring tags in the cluster.
The second interface consists of a 2D-visualisation of the k-Nearest Neighbor Graph, where colors are used for representing clusters as shown in Figure \ref{fig:src_2d_visu}. Sounds can be played by hovering the mouse on the nodes.
Moreover, clicking on a node will highlight its neighbors in order to ease neighborhood exploration. 

\begin{figure*}
 \centering
 \includegraphics[width=0.93\textwidth]{src_facet_search2.png}
 \caption{Page displaying the result of the query \textit{glass} of the \textit{cluster \#1}. Clicking on a cluster facet on the right applies a cluster filter. Three labels are shown for each cluster, together with the number of sounds they contain.}
 \label{fig:src_facet}
\end{figure*}

\begin{figure*}
 \centering
 \includegraphics[width=0.93\textwidth]{src_2d_visu2.png}
 \caption{The graphical 2D visualisation of sounds retrieved with the query \textit{guitar}. Each circle represents a sound. Placing the mouse on one will play the associated sound. Clicking on it displays some information at the top of the screen and highlights neighbor nodes.}
 \label{fig:src_2d_visu}
\end{figure*}

==> ICMR 20 - Search Result Clustering in Collaborative Sound Collections(1)/S4_evaluation1.tex <==
In this section we show some comparative performance results of our approach using the different sets of features previously described.
We perform two different evaluations: one using internal validation and another using external validation.
For the first one, we propose to leverage information from an existing sound sharing website to automatically evaluate the clustering performances at scale.
We then perform a standard evaluation which uses ground truth labels taken from manually annotated datasets.
One of the goals to perform these two evaluations is to validate that our first evaluation that does not require known ground truth labels is adequate for comparing the performance of different clustering methods.


\subsection{Internal Validation}

We consider the Freesound database as a use case and we perform clustering on the search results of popular queries submitted by real users of the platform. We focus only on sounds with duration from 0 to 10 seconds.
For a quantitative evaluation, we make use of the sounds' metadata that is provided by the creator of the content in the Freesound platform.
%

Evaluating a clustering automatically is a complicated task, and there are different types of metrics that can be used~\cite{manning2010introduction}.
Some of them are referred as internal metrics, and they are used when no ground truth label is known~\cite{liu2010understanding}.
The Calinski-Harabasz Index (CHI)~\cite{calinski1974dendrite} evaluates the cluster validity based on the average between- and within-cluster sum of squares as shown in this equation:
\begin{equation}
CH(k)=[B(k) / W(k)] × [(n - k)/(k - 1)]
\end{equation}
Where $n$ corresponds to the number of data points, $k$ to the number of clusters, $W(k)$ to the within cluster variation and $B(k)$ to the between cluster variation.

% TODO: explain better here
%
% It seems to be a reasonable choice since we want here get an evaluation that is robust to outliers (compared to Silouhet coeff)
%
Instead of calculating this metric using the audio features used for clustering, we make use of the user-provided tags associated with the audio content as an external information.
This allows us to evaluate the overall quality of a clustering, from a semantic perspective.
From the tags associated to the content, we derive a feature using a Vector Space Model representation~\cite{salton1989automatic}.
This feature is a high-dimentional sparse vector where a value of 1 in one dimension refers to the presence of a specific tag.
We only consider the 5000 tags that occur the most in the overall Freesound collection.
We then reduce the size of this vector to 100, by applying Latent Semantic Analysis, which can capture synonymy relations~\cite{deerwester1990indexing}.
%
% Results using this metric are presented in Table \ref{tab:evaluation} and \ref{tab:evaluation2}.
Due to the nature of tags, the validity metric we use is not always accurate.
In order to mitigate this problem, we average this metric on clusterings performed on the results of the 1000 most popular queries in Freesound.
In total, approximately 80k different sounds were used in this evaluation.
Figure \ref{fig:src_eval_tags} represents the evaluation pipeline.
%
% MOVE TO 4.3?
The statistics are presented in Table \ref{tab:evaluation}.
%
% Table \ref{tab:evaluation2} shows the values of the modularity and validity index of the clusterings performed on the results of a few popular selected queries.


\begin{figure}
 \centering
 \includegraphics[width=\columnwidth]{SRC_eval_features.png}
 \caption{Diagram representing the steps of our internal evaluation making use of user-provided tags. The Calinski-Harabasz Index is calculated between the labels corresponding to the obtained clusters and the features derived from the sound tags. This evaluation is performed on the results of the 1000 most popular queries performed by Freesound users.}
 \label{fig:src_eval_tags}
\end{figure}

\subsection{External Validation}
As an additional evaluation, we also make use of an
external validation metrics, which relies on known ground truth labels. 
We exploit data gathered within Freesound Annotator
% \footnote{\url{https://annotator.freesound.org/}}
~\cite{fonseca2017freesound} to construct 44 datasets comprising in total around 30k sounds and 215 different labels. 
Labels are drawn from the AudioSet Ontology~\cite{gemmeke2017audio}, which consists of a hierarchical taxonomy of 635 sound-related categories.
In our experiment, a dataset consists of one node in the taxonomy, and its labels are its direct children. 
This creates datasets of different sizes and with different levels of specificity. 
For instance, one broad dataset corresponds to natural sounds, containing the \textit{water}, \textit{wind}, \textit{thunderstorm} and \textit{fire} classes.
A more specific one contains only water sounds, with the \textit{rain}, \textit{stream}, \textit{steam}, \textit{waterfall}, \textit{gurgling}, and \textit{ocean} classes.
All the datasets contain sounds with a duration lower than 10 seconds and most of them contain only one salient source, which mitigates the inconvenience of using a statistical aggregation over the frame-based features.
%
Among the popular metrics used for comparing dataset partitions, the literature suggests that Adjusted Mutual Information (AMI) score~\cite{vinh2010information} is suited when the reference clustering (ground truth) is unbalanced and there exist small clusters~\cite{romano2016adjusting}.
This corresponds often to what we find in collaborative collections where the content is inconsistently distributed in terms of type and nature.
For evaluating the different sets of features with the different features, we perform clustering on the datasets and measure the similarity between the real partition (given by the ground truth labels) and the one given by the clustering methods by computing the Mutual Information score adjusted for chance (AMI), calculated as following:
\begin{equation}
AMI(U, V) = \frac{MI(U, V) - E\{MI(U, V)\}}{max\{H(U), H(V)\} - E\{MI(U, V)\}}
\end{equation}
\begin{equation}
MI(U, V) = \sum_{i} \sum_{j} P(i, j) \log(\frac{P(i, j)}{P(i) P(j)})
\end{equation}
Where $U$ and $V$ are the two partitions to compare, $H(U)$ and $H(V)$ their associated entropy. $P(i)$ and $P(j)$ the probabilities that a point belongs to cluster $U_i$ or $V_j$ respectively, $P(i,j)$ the probability that a point belongs to both cluster $U_i$ and $V_j$ from $U$ and $V$ respectively, and $E\{MI(U, V)\}$ corresponds to the expected mutual information between two random clusterings.
The Mutual Information metric (MI) quantifies the information shared by the two partitions and therefore can be used as a clustering similarity measure.
When adjusted for chance, the metric takes a value of 1 for two identical partitions and the value of 0 for two randomly dissimilar partitions.
%
% MOVE THAT TO 4.3?
Table \ref{tab:scores} shows some statistics of this score for the different audio features.


\subsection{Results}
% ADD ANALYSIS OF THE RESULTS
% VALIDATE OUR AUTOMATIC ~INTERNAL EVALUATION
In both evaluations, AudioSet embeddings lead to the best clustering performance.
This shows that novel deep learning approaches can produce semantically meaningful features that outperform traditional hand-crafted features for the unsupervised classification of sounds.
There is not any meaningful difference when applying manual feature selection over hand-crafted features (F1) motivated by results taken from the literature compared to using a large set of lowlevel features (F2).
%

Our approach for discarding low quality clusters using the confidence measure described in Section 3.3 shows little but consistent improvement with all the features in both experiments.
%

Another conclusion is that our proposed internal validation which makes use of accompanying tags provided by the users of the platform can give similar results as an external validation using ground-truth labels.
This provides a valuable framework for evaluating clustering algorithms in existing multimedia collections at scale, without needing to manually annotate a large amount of data.

% For the rest of this work, we use the AudioSet embeddings in our clustering engine.

% TABLE RESULT
\begin{table}
\small
 \begin{center}
 \begin{tabular}{l|cc|cc}
  \toprule
  \multirow{3}{*}{Features} & \multicolumn{4}{c}{CHI} \\
  & \multicolumn{2}{c}{no pruning} & \multicolumn{2}{c}{pruning} \\
  & mean & std & mean & std \\
  \midrule
  F1    & 3.36 & 5.87 & 3.88 & 7.25 \\
  F2    & 3.44 & 6.37 & 3.86 & 7.07 \\
  F3    & \textbf{4.29} & 6.82 & \textbf{5.29} & 11.06 \\
  \bottomrule
 \end{tabular}
\end{center}
 \caption{Clustering validity score (Calinski-Harabasz Index) using the different feature sets. Mean and standard deviation is calculated on the performance of the clustering of the results from the top 1000 most popular queries in Freesound. The pruning column corresponds to the validity score when discarding the cluster with the lowest confidence score defined in Section 3.3.}
 \label{tab:evaluation}
\end{table}

% TABLE RESULT
\begin{table}
\small
 \begin{center}
 \begin{tabular}{l|cc|cc}
  \toprule
  \multirow{3}{*}{Features} & \multicolumn{4}{c}{AMI} \\
  & \multicolumn{2}{c}{no pruning} & \multicolumn{2}{c}{pruning} \\
  & mean & std & mean & std \\
  \midrule
  F1    & 0.16 & 0.08 & 0.18 & 0.10 \\
  F2    & 0.15 & 0.09 & 0.16 & 0.12 \\
  F3    & \textbf{0.20} & 0.10 & \textbf{0.21} & 0.11 \\
  \bottomrule
 \end{tabular}
\end{center}
 \caption{Average performance (AMI) across the different dataset with the different features. An AMI close to 0 corresponds to a random partition while perfect matches gives 1 AMI. The pruning column corresponds to the performance when discarding the cluster with the lowest confidence score defined in Section 3.3.}
 \label{tab:scores}
\end{table}

% \setlength{\tabcolsep}{0.2em}
% \begin{table}
% \small
%  \begin{center}
%  \begin{tabular}{l|cc|cc|cc}
%   \toprule
%   \multirow{2}{*}{Queries} & \multicolumn{2}{c}{F1} & \multicolumn{2}{c}{F2} & \multicolumn{2}{c}{F3} \\
%   & CHI &modularity & CHI & modularity & CHI & modularity \\
%   \midrule
%   wind      & 7.36  & 0.71  & 10.50 & 0.56 & 6.00  & 0.52 \\
%   music     & 2.75  & 0.84  & 12.48 & 0.45 & 18.01 & 0.54 \\
%   guitar    & 7.00  & 0.78  & 14.86 & 0.69 & 18.09 & 0.65 \\
%   jingle    & 5.20  & 0.83  & 20.82 & 0.49 & 17.29 & 0.42 \\
%   piano     & 6.67  & 0.84  & 9.26  & 0.18 & 24.72 & 0.66 \\
%   string    & 12.17 & 0.76  & 8.96  & 0.54 & 15.47 & 0.67 \\
%   \bottomrule
%  \end{tabular}
% \end{center}
%  \caption{Clustering validity score (Calinski-Harabasz Index) using the different feature sets when clustering the results of different popular queries in Freesound.}
%  \label{tab:evaluation2}
% \end{table}


% SMALL CONCLUSION SAYING THAT AUDIOSET SEEM BETTER AND WE USE ADOPT THEM FOR OUR SRC APPROACH

% \balance{}

==> ICMR 20 - Search Result Clustering in Collaborative Sound Collections(1)/S5_qualitative_evaluation.tex <==
\subsection{Examples}
We qualitatively evaluate our approach by manually inspecting the clustering results performed on several selected queries.
% We qualitatively evaluate our approach on a few examples of clustering.
For this purpose, we make available to the reader an interface that displays a graph representation of the sounds as seen in Figure \ref{fig:graph}.
The interface is available from a web browser at: \url{https://graph-based-clustering-ismir.github.io/}. % UPDATE LINK; SETUP REPO
% we use an interface that displays nodes and edges in a two-dimensional space using a force layout, and allows to listen to the sounds, as shown in Figure \ref{fig:graph}.
% The clustered graphs for some selected queries shown are made available from a browser at this address: \url{https://graph-based-clustering-ismir.github.io/}. % UPDATE LINK; SETUP REPO
In this page, buttons at the top allow you to choose the query and the features used for the graph creation and its partition.
When hovering a node with the mouse, the corresponding sound is played, and the name of the audio clip and its tags are displayed.
The colors correspond to the assigned clusters.
You can zoom in and out using the mouse wheel, and move in the space by dragging.
In the following we provide a concise discussion around some observed interesting clustering results.

\begin{figure}
 \centering
 \includegraphics[width=\columnwidth]{src_graph_qualitative_eval.png}
 \caption{Visualisation of the clustered graph for the query "guitar" using AudioSet features (F3). The graph for different search query results can be explored from a browser at this url: \url{https://graph-based-clustering-ismir.github.io/}}
 \label{fig:graph}
\end{figure}

% \subsection{Discussion}
% In this section we discuss our approach by making use of both quantitative and qualitative evaluations.
% We organise our discussion around important themes and aspects that a clustering engine should satisfy for being integrated as a complement of a traditional search engine.

\vspace{1.1pt}
\textbf{Capturing semantic concepts.}
One important ability that the clustering method should have is to capture semantic concepts.
This is particularly useful when search results are corrupted with sounds that correspond for instance to another instrument and were retrieved because the textual description provided by the uploader of the sounds, contained wrong terms.
%
% A similarity is, to some extent, reflected in the tag-based feature that we use for evaluating the model.
% Features trained on AudioSet (F3) clearly show better performance than the acoustic feature sets (F1 and F2).
%
When using the AudioSet features (F3),
hat are trained using a large dataset containing millions of items, with more than 600 categories,
we observe that their representation ability go beyond these considered semantic categories. % rephrase
For instance, they are also able to group together different perceptually similar sounds, created from peculiar uses of a guitar (strings brushing, string drop and metal scratch) which are not part of the AudioSet categories.
Similarly, for the "piano" query, toy or detuned piano sounds are clustered together. % maybe add screenshot?
This motivates the use of supervised approaches for learning features with annotated data.
Even if the categories do not cover all the necessary concepts involved for describing all the specific aspects of the content.

\vspace{1.1pt}
\textbf{Context dependent similarity.} 
A similarity notion between objects is in practice difficult to establish, since it is often context dependent.
In the case of sound retrieval, some of context is given by the query the user submits to the search engine.
In the case of the "music" query, it is reasonable to assume that string instruments or all musical instruments are considered similar and can be grouped in the same cluster.
However, if the context is a particular instrument such as "guitar", the similarity consideration would need to be adapted. 
Approaches based on k-nearest neighbors are particularly suited for this, since they don't use any threshold for assuming that two things are considered similar within a collection. 
As an example, with the AudioSet features, the clusters obtained with the "music" query groups together guitars and cellos. 
However, for the "string" query, different types of string instruments are often placed in distinct clusters.

\vspace{1.1pt}
\textbf{Ambiguous queries.}
% Lexical ambiguity is a fundamental problem is natural language processing.
% When, submitting an ambiguous query to a search engine, 
Submitting queries containing polysemic terms to a search engine will result in having items from the different meanings mixed in the same ranked list.
The same problem will occur when queries express a vague and broad need.
% broad meaning are used.
Clustering these results should divide these results into different clusters, in order to provide an overview of the different topics covered by the query.
% To be beneficial to users, the different clusters should contain the results corresponding to different possible meanings covered by the user query.
As an example, "jingle" can refer to, a light ringing sound, or a short music tune designed to be easily remembered.
%
Additionally, "string" can refer to many different string musical instruments, or to sounds produced with a casual string.
Separating these different semantic topics in different clusters is what would be expected from a clustering engine, since these concepts are semantically and perceptually quite different.
%
Music is an example of a broad query which will retrieve many different types of content: musical loops, single instruments, and so on.
% ambiguous cases are the queries that reflect a vague and broad need, such as "music". 
% In this sort of cases, we expect the system to provide an overview of the different topics covered by the broad query.
%
In order to obtain such a result, the features used for the clustering should be able to discriminate sounds from the different topics. 
The clustering method which uses AudioSet feature satisfies this disambiguation requirement, where sounds from the different topics often appear in different clusters.
% Again, the ability of pre-traing embeddings with large datasets using a lot of categories shows it potential.

% \vspace{1pt}
% \textbf{Confidence measure.} 
% One of the objectives of this work is to investigate the use of cluster quality metrics derived directly from the graph representation and its partition.
% Table \ref{tab:evaluation} shows the averaged performance of the clustering method for different sets of features on results from the 1000 most popular queries in Freesound.
% Simply discarding the cluster with the lower confidence score defined in Section 3.3 improves significantly the clustering validity score (Calinski-Harabasz Index) when using F2 and F3 feature sets.
% %
% In addition, table \ref{tab:evaluation2} shows the modularity of the graph partitions on different query results. 
% A low modularity value is often associated to a low validity score, which asserts the reliability of using internally derived confidence measure for discarding bad partitions.
% This result provides some useful insights on ways to validate some individual clusters that are worth presenting to the user.
% Moreover, it allows us to combine the results of different clustering performed on the data collections.
% It could for instance enable the automatic creation of faceted navigation systems, where a user can narrow down search results by applying filters on different discovered aspects~\cite{tunkelang2009faceted}.


% \vspace{1pt}
% \textbf{Acoustic features.}
% Despite the effort done in selecting features (F1) that were successful for classification tasks in different audio-related domains, their performances in our unsupervised classification of search results is quite low.
% However, when aggregating a bigger set of features (F2), the clusters obtained show better compactness and distinctiveness. 
% One reason could be that the small set of selected feature is not able to generalize to the diversity of the search results.
% %
% Another intuition is that the feature reduction step that we perform (i.e., Principal Component Analysis), is not adequate for selecting suitable features that can differentiate the types of sounds.
% Instead, one solution would be to apply a supervised feature selection method on the aggregated feature statistics~\cite{zhao2007spectral}.
% Using datasets involving a large amount of categories are appropriate for describing the wide range of sound types present in online collections.
% As an example, datasets using the categories drawn from the AudioSet Ontology are applicable~\cite{gemmeke2017audio, fonseca2017freesound}.
% % However, the aggregation of many sometimes redundant features provided better performance.
% % this does not motivate to do more manual feature selection
% Another alternative that could give interesting results for the user, would consists in using less acoustic features.
% For instance, using lowlevel features that are related to perceptual attributes of sounds, such as spectral centroïd, could provide, in a limited context such as "guitar", clusters that reflect essential characteristics of the sounds.


==> ICMR 20 - Search Result Clustering in Collaborative Sound Collections(1)/S6_evaluation2.tex <==
In this section, we present our user-centered design process on the development of an interface for browsing sounds from large databases using the proposed clustering engine.
In this experiment, we use the AudioSet features (F3), which achieved the best performance in our comparative performance evaluation.
We use our interface prototypes as \textit{technology probes} to observe their use in a real context, to evaluate their functionalities and to inspire new ideas~\cite{hutchinson2003technology}. 

\subsection{Methodology}
We performed experiments with 4 users that are experienced with audio and sound design tasks, which is sufficient for detecting a large amount of usability problems~\cite{Nielsen_2000_5UserTest}.
All the participants were presented with the two searching tools (clustering facets filtering and 2D-visualisation) presented in Section 3.4.
The task consisted in gathering all the audio content needed in order to build the soundtrack of a short video, available at: \url{https://vimeo.com/333837958}. This video was chosen because it was short but presenting a lot of variety of elements to sonify.
The original sound was removed from the video.
Some guidelines were shown to the participants, together with verbal explanations given by the examinator who was present during the entire experiment.
At the end of the task, they were provided with a questionnaire containing some usability and engagement questions.
Finally, semi-structured interviews were carried out, including open-ended questions as well as specific questions related to observed behaviors during the performance of the task.
This enables discussion using thematic analysis in order to identify emerging themes from participants' answers.

\subsection{Results and discussion}

All the participants started by watching the video and noting down the concepts they would then look for within the audio collections.
Then, they started to use the search engine to look for the identified concepts needed for sonifying the video.
After entering a query, users often had a quick look at the top results.
They explained that it allowed them to figure out if the content retrieved was the one they were expecting. 
They then had the choice to either reformulate their query, or explore the retrieved results.
%
% REFORMULATE
They found particularly useful the labels associated with each clusters in order to identify what kind of sounds were present in the results and what type of content each cluster contained.
% each cluster was corresponding to. 
%
They were either applying a cluster filtering to then browse the results in the retrieved sounds, or they would use terms from the cluster labels to reformulate their query.

However, some participants complained that the cluster labels were sometimes inappropriate, because they contained too broad concepts, or they were very similar for different clusters.
In these cases, it was hard to understand what type of content each cluster contained.
Nevertheless, the 2D-visualisation was then particularly helpful.
The participants were often listening to many sounds in a short amount of time thanks to the the fact that they only needed to hover the mouse on different nodes to start hearing some sounds. 
Whereas in the flat ranked list, they would have to manually trigger the players by clicking many times.
In the 2D-visualisation, their strategy was to first listen to a few dispersed sounds to quickly get an idea of how the sounds were organised in the space and what type of content was present in each cluster. 
Then, they would start exploring specific regions of interest, until they satisfy their need by retrieving one or several relevant sounds.
%
In addition, the users were often searching in a sound’s neighborhood. 
They explained that they wanted to find some slightly different variations of a relevant sound they already located.
%
However, understanding what the dimensions were capturing in the space was difficult.
The graph representation of the sound results was failing to reflect timbral characteristics of the sounds in a clear way.
%
Moreover, even if the graph was presenting a clear structure, it was not easy to understand to what it was corresponding to and to locate all the relevant content.
As a solution, a participant wanted to be able to select any retrieved sound from the ranked list and locate it in the 2D-visualisation.
This way, he explained that he could easily switch from one interface to the other, allowing him to efficiently combine the two interaction approaches.
% From a relevant sound located in the flat ranked list, start from an interesting location for then exploring the graph.
% Furthermore, when switching to the 2D-visualisation, the user is not presented with cluster indexes or labels anymore. 
% Some participants explained that after identifying interesting clusters, they would like to locate them in the 2D-visualisation.

The clustering engine was not very beneficial when the participants were using precise queries containing multiple words. 
They explained that in the context of sound design, they often know exactly what they need. And therefore they were often able to formulate a precise text query retrieving very specific content.
However, one drawback is that sounds that would not present the query terms as metadata would not be retrieved.
A solution to deal with bad recall performance of the system would be to use the audio-based representation to expand the retrieved results with sounds that are similar to the one retrieved.
In its current state, the prototype only applies clustering on the retrieved results, but does not include sounds that could have been relevant, but were missed to be retrieved by the text-based search engine.
Using the audio-based features for expanding the retrieved results would be interesting to study for queries that retrieved very few results. 
% Again using the graph for visualising similar sounds could help with retrieving sounds that were not necessarily retrieved by the text-based search engine. 

Some participants criticised the fact that the 2D-visualisation did not provide any representation of the waveform or any time-related information regarding the audio clips.
This made it hard to explore some results, as many of the users actively use waveforms in order to identify for instance if a foreground sound would appear at some time in the audio clip.
For that reason, in the 2D-visualisation, many participants were skipping some audio clips because the main acoustic event was not starting at the beginning of the clip.
Moreover, some participants said that they often use the waveform representation to assess some characteristics of the sounds, such as its dynamics, or the level of background noise present in the audio clip. 
Displaying the waveform with a time progression cursor of the current sound being played is therefore a key feature that would make the 2D-visualisation more useful and attractive.

Finally, in its current state, the clustering algorithm is able to discover distinctive and coherent groups in search results for many given queries.
However, in some cases, the quality of the clustering is still low, which made some users wasting time exploring bad clusters. 
Moreover, they explained that spending time exploring non-relevant clusterings could make them lose trust in the system, and therefore make them not use it again.
It was discussed in the interview the idea of reporting an estimate of the quality of the clustering, so that the user would be aware of its poor result and would be more confident while using the system. 
Using a confidence measure such as the one proposed in Section 3.3 could be a solution, or using directly the modularity of the graph partition.
Our evaluation of the strategy for discarding low quality clusters in Section 4 indicates that such measures can reflect, to some extent, the quality of the clustering.
% This would be interesting to test with users, for instance by showing a quality score for a clustering or for each clusters.

% \textbf{SRC can organize results by sub-topics of the query.}
% When searching for sounds, the Search Result Clustering prototype sometimes guided the users in reformulating their query using terms from the cluster labels. 
% Also, they were sometimes using tags from sounds they were listening. 
%This corresponds to what is described in the web search engine literature for SRC.

% \textbf{Enable to reformulate the query.}
% When the clustering is able to discover some distinctive high quality clusters, it is important to provide some labels that reflect some semantic properties of the clusters. This labels are useful in order to make the user understand what type of sounds and covered in a cluster and can also be used for reformulating the query.

% \textbf{Find variation of a sound.}
% In the 2D visualisation, users were often searching in a sound’s neighborhood. They explained that they wanted to find some slightly different variations of a relevant sound they already located. Interestingly, one participant wanted to be able to select a sound from the flat ranked list to set is as “context” in the 2D plan. This can be an alternative to the flat list returned when using the “similar sound” feature in Freesound.

% \textbf{Faster exploration with the visualisation tool.}
% In the 2D visualisation, users were often exploring many sounds in a short time. For large graphs, they typically try to get an idea of what sort of sounds are present in the plan by listening to a few dispersed sounds. Then they start to explore specific regions of interest until they satisfy their need with one or several relevant sounds.

% \textbf{Sound designers often know exactly what they want and use precise queries.}
% During the experiment, most of the participants used precise query containing multiple words. They explained that in the context of sound design, they often know exactly what they want. One drawback is that many sounds in collaborative collections might not be described in an exhaustive way, with precise keywords that the user used in his query. Thus, some relevant sounds might not be retrieved.

% \textbf{Clusters don’t allow to explore across timbres in a controllable way.}
% Some users said that they were trying to understand what dimensions were captured by the system. For instance, in the 2D visualisation, they were trying to understand if one geometric dimension or area was corresponding to a specific timbre characteristics, such as brightness for instance. The graph representations of the sound results were not able to capture these desired dimension in a clear way.

% \textbf{Users often check first results to quickly judge if it is good enough to continue browsing the results.}
% Most of the participants started to explore the results from the flat list. One participant argued that he wanted to be confident about the types of sounds that were in the results before continuing searching using the clustering functionalities. 

% \textbf{Many users rely on the waveform for exploring through time and accessing characteristics of audio clips.}
% The 2D visualisation received a lot of complaints regarding the fact that no visualisation of the waveform or neither time information was provided. This made it harder to explore the sounds. Some users make a strong use of the waveform in order to judge if a foreground sound is going to play. Others said that they even use it in order to access some characteristics of the background sounds present in audio clips. Moreover, in the visualisation, many participants were skipping some sounds because the main acoustic event present in the clip was not starting at the beginning of the clip.

%Queries are often adjusted after results inspection

% \textbf{Bad accuracy on the clustering can make user loose time and confidence in the system.}
% In it current state, the clustering algorithm is able to discover distinctive and coherent groups in the search results. However, for some queries, the quality of the clustering is poor, which made some users spend time randomly exploring the results. It was discussed in the interview the idea of reporting an estimate of the quality of the clustering, so that the user would have more confidence in the system. One participant proposed that users of the platform could rate the clustering, which would be inadequate given that the clustering results will evolve in time due to the constant growth of the collection.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> S5_qualitative_evaluation.tex <==
\subsection{Examples}
We qualitatively evaluate our approach by manually inspecting the clustering results performed on several selected queries.
% We qualitatively evaluate our approach on a few examples of clustering.
For this purpose, we make available to the reader an interface that displays a graph representation of the sounds as seen in Figure \ref{fig:graph}.
The interface is available from a web browser at: \url{https://graph-based-clustering-ismir.github.io/}. % UPDATE LINK; SETUP REPO
% we use an interface that displays nodes and edges in a two-dimensional space using a force layout, and allows to listen to the sounds, as shown in Figure \ref{fig:graph}.
% The clustered graphs for some selected queries shown are made available from a browser at this address: \url{https://graph-based-clustering-ismir.github.io/}. % UPDATE LINK; SETUP REPO
In this page, buttons at the top allow you to choose the query and the features used for the graph creation and its partition.
When hovering a node with the mouse, the corresponding sound is played, and the name of the audio clip and its tags are displayed.
The colors correspond to the assigned clusters.
You can zoom in and out using the mouse wheel, and move in the space by dragging.
In the following we provide a concise discussion around some observed interesting clustering results.

\begin{figure}
 \centering
 \includegraphics[width=\columnwidth]{src_graph_qualitative_eval.png}
 \caption{Visualisation of the clustered graph for the query "guitar" using AudioSet features (F3). The graph for different search query results can be explored from a browser at this url: \url{https://graph-based-clustering-ismir.github.io/}}
 \label{fig:graph}
\end{figure}

% \subsection{Discussion}
% In this section we discuss our approach by making use of both quantitative and qualitative evaluations.
% We organise our discussion around important themes and aspects that a clustering engine should satisfy for being integrated as a complement of a traditional search engine.

\vspace{1.1pt}
\textbf{Capturing semantic concepts.}
One important ability that the clustering method should have is to capture semantic concepts.
This is particularly useful when search results are corrupted with sounds that correspond for instance to another instrument and were retrieved because the textual description provided by the uploader of the sounds, contained wrong terms.
%
% A similarity is, to some extent, reflected in the tag-based feature that we use for evaluating the model.
% Features trained on AudioSet (F3) clearly show better performance than the acoustic feature sets (F1 and F2).
%
When using the AudioSet features (F3),
hat are trained using a large dataset containing millions of items, with more than 600 categories,
we observe that their representation ability go beyond these considered semantic categories. % rephrase
For instance, they are also able to group together different perceptually similar sounds, created from peculiar uses of a guitar (strings brushing, string drop and metal scratch) which are not part of the AudioSet categories.
Similarly, for the "piano" query, toy or detuned piano sounds are clustered together. % maybe add screenshot?
This motivates the use of supervised approaches for learning features with annotated data.
Even if the categories do not cover all the necessary concepts involved for describing all the specific aspects of the content.

\vspace{1.1pt}
\textbf{Context dependent similarity.} 
A similarity notion between objects is in practice difficult to establish, since it is often context dependent.
In the case of sound retrieval, some of context is given by the query the user submits to the search engine.
In the case of the "music" query, it is reasonable to assume that string instruments or all musical instruments are considered similar and can be grouped in the same cluster.
However, if the context is a particular instrument such as "guitar", the similarity consideration would need to be adapted. 
Approaches based on k-nearest neighbors are particularly suited for this, since they don't use any threshold for assuming that two things are considered similar within a collection. 
As an example, with the AudioSet features, the clusters obtained with the "music" query groups together guitars and cellos. 
However, for the "string" query, different types of string instruments are often placed in distinct clusters.

\vspace{1.1pt}
\textbf{Ambiguous queries.}
% Lexical ambiguity is a fundamental problem is natural language processing.
% When, submitting an ambiguous query to a search engine, 
Submitting queries containing polysemic terms to a search engine will result in having items from the different meanings mixed in the same ranked list.
The same problem will occur when queries express a vague and broad need.
% broad meaning are used.
Clustering these results should divide these results into different clusters, in order to provide an overview of the different topics covered by the query.
% To be beneficial to users, the different clusters should contain the results corresponding to different possible meanings covered by the user query.
As an example, "jingle" can refer to, a light ringing sound, or a short music tune designed to be easily remembered.
%
Additionally, "string" can refer to many different string musical instruments, or to sounds produced with a casual string.
Separating these different semantic topics in different clusters is what would be expected from a clustering engine, since these concepts are semantically and perceptually quite different.
%
Music is an example of a broad query which will retrieve many different types of content: musical loops, single instruments, and so on.
% ambiguous cases are the queries that reflect a vague and broad need, such as "music". 
% In this sort of cases, we expect the system to provide an overview of the different topics covered by the broad query.
%
In order to obtain such a result, the features used for the clustering should be able to discriminate sounds from the different topics. 
The clustering method which uses AudioSet feature satisfies this disambiguation requirement, where sounds from the different topics often appear in different clusters.
% Again, the ability of pre-traing embeddings with large datasets using a lot of categories shows it potential.

% \vspace{1pt}
% \textbf{Confidence measure.} 
% One of the objectives of this work is to investigate the use of cluster quality metrics derived directly from the graph representation and its partition.
% Table \ref{tab:evaluation} shows the averaged performance of the clustering method for different sets of features on results from the 1000 most popular queries in Freesound.
% Simply discarding the cluster with the lower confidence score defined in Section 3.3 improves significantly the clustering validity score (Calinski-Harabasz Index) when using F2 and F3 feature sets.
% %
% In addition, table \ref{tab:evaluation2} shows the modularity of the graph partitions on different query results. 
% A low modularity value is often associated to a low validity score, which asserts the reliability of using internally derived confidence measure for discarding bad partitions.
% This result provides some useful insights on ways to validate some individual clusters that are worth presenting to the user.
% Moreover, it allows us to combine the results of different clustering performed on the data collections.
% It could for instance enable the automatic creation of faceted navigation systems, where a user can narrow down search results by applying filters on different discovered aspects~\cite{tunkelang2009faceted}.


% \vspace{1pt}
% \textbf{Acoustic features.}
% Despite the effort done in selecting features (F1) that were successful for classification tasks in different audio-related domains, their performances in our unsupervised classification of search results is quite low.
% However, when aggregating a bigger set of features (F2), the clusters obtained show better compactness and distinctiveness. 
% One reason could be that the small set of selected feature is not able to generalize to the diversity of the search results.
% %
% Another intuition is that the feature reduction step that we perform (i.e., Principal Component Analysis), is not adequate for selecting suitable features that can differentiate the types of sounds.
% Instead, one solution would be to apply a supervised feature selection method on the aggregated feature statistics~\cite{zhao2007spectral}.
% Using datasets involving a large amount of categories are appropriate for describing the wide range of sound types present in online collections.
% As an example, datasets using the categories drawn from the AudioSet Ontology are applicable~\cite{gemmeke2017audio, fonseca2017freesound}.
% % However, the aggregation of many sometimes redundant features provided better performance.
% % this does not motivate to do more manual feature selection
% Another alternative that could give interesting results for the user, would consists in using less acoustic features.
% For instance, using lowlevel features that are related to perceptual attributes of sounds, such as spectral centroïd, could provide, in a limited context such as "guitar", clusters that reflect essential characteristics of the sounds.

